Interpretable machine learning for finding intermediate-mass black holes

Definitive evidence that globular clusters (GCs) host intermediate-mass black holes (IMBHs) is elusive. Machine learning (ML) models trained on GC simulations can in principle predict IMBH host candidates based on observable features. This approach has two limitations: first, an accurate ML model is expected to be a black box due to complexity; second, despite our efforts to realistically simulate GCs, the simulation physics or initial conditions may fail to fully reflect reality. Therefore our training data may be biased, leading to a failure in generalization on observational data. Both the first issue -- explainability/interpretability -- and the second -- out of distribution generalization and fairness -- are active areas of research in ML. Here we employ techniques from these fields to address them: we use the anchors method to explain an XGBoost classifier; we also independently train a natively interpretable model using Certifiably Optimal RulE ListS (CORELS). The resulting model has a clear physical meaning, but loses some performance with respect to XGBoost. We evaluate potential candidates in real data based not only on classifier predictions but also on their similarity to the training data, measured by the likelihood of a kernel density estimation model. This measures the realism of our simulated data and mitigates the risk that our models may produce biased predictions by working in extrapolation. We apply our classifiers to real GCs, obtaining a predicted classification, a measure of the confidence of the prediction, an out-of-distribution flag, a local rule explaining the prediction of XGBoost and a global rule from CORELS.

==> false_negative_anchors.tex <==
\begin{tabular}{rlrr}
\hline
    & anchor                                                                                                          &   precision &   coverage \\
\hline
  0 & ['3365.87 \ensuremath{<} HRT \ensuremath{<}= 5368.92', 'TVL \ensuremath{<}= 73782.70', 'CVD \ensuremath{<}= 6.38', 'CSB \ensuremath{<}= 6400.19', 'OCR \ensuremath{<}= 1.45', 'OHLR \ensuremath{<}= 4.92'] &    0.944853 & 0.0738636  \\
  1 & ['HRT \ensuremath{>} 5368.92', 'CSB \ensuremath{<}= 2027.60']                                                                             &    0.976247 & 0.163961   \\
  2 & ['TVL \ensuremath{<}= 6516.13', 'CVD \ensuremath{<}= 3.51']                                                                               &    0.976744 & 0.25       \\
  3 & ['OCR \ensuremath{>} 0.78', 'HRT \ensuremath{>} 1323.51', 'CVD \ensuremath{<}= 6.38', 'OHLR \ensuremath{>} 2.12', 'TVL \ensuremath{<}= 73782.70']                                &    0.901768 & 0.284903   \\
  4 & ['HRT \ensuremath{>} 5368.92', 'OHLR \ensuremath{>} 4.92', 'CVD \ensuremath{<}= 6.38']                                                                 &    0.964602 & 0.146104   \\
  5 & ['HRT \ensuremath{>} 5368.92', 'CSB \ensuremath{<}= 2027.60']                                                                             &    0.961276 & 0.163961   \\
  6 & ['HRT \ensuremath{>} 5368.92', 'CSB \ensuremath{<}= 6400.19']                                                                             &    0.908894 & 0.221591   \\
  7 & ['HRT \ensuremath{>} 5368.92', 'OCR \ensuremath{>} 1.45', 'CVD \ensuremath{>} 6.38', 'OHLR \ensuremath{<}= 4.92']                                                   &    0.957364 & 0.00730519 \\
  8 & ['HRT \ensuremath{>} 5368.92', 'OHLR \ensuremath{>} 4.92']                                                                                &    0.971264 & 0.178571   \\
  9 & ['HRT \ensuremath{>} 3365.87', 'OCR \ensuremath{<}= 0.78', '2.12 \ensuremath{<} OHLR \ensuremath{<}= 2.95']                                                         &    0.934659 & 0.0551948  \\
 10 & ['HRT \ensuremath{>} 5368.92', 'OHLR \ensuremath{>} 4.92']                                                                                &    0.964126 & 0.178571   \\
\hline
\end{tabular}

==> false_negatives.tex <==
\begin{tabular}{rrrrrrr}
\hline
      &        HRT &       TVL &      CVD &      CSB &      OCR &    OHLR \\
\hline
   33 &  3960.75   &  48638.3  &  6.36992 &  3619.96 & 0.893196 & 3.23121 \\
   84 &  6479.46   &  40964.9  &  2.80751 &  1023.3  & 1.4509   & 5.99196 \\
  119 &    29.6169 &   4037.29 &  3.24157 &   590.23 & 1.96383  & 1.16389 \\
  680 &  3178.53   &  72723.6  &  3.93017 &  5524.64 & 1.0461   & 2.4593  \\
  717 &  7779.41   &  73973.7  &  3.14057 &  2172.11 & 1.4101   & 5.08386 \\
  890 &  7547.65   &  77113.6  &  4.38514 &  1962.44 & 1.6583   & 4.90466 \\
 1026 &  6428.01   &  92741.2  &  6.79258 &  4010.07 & 1.25359  & 3.78693 \\
 1034 &  8306.58   & 118080    &  7.08831 &  4441.48 & 1.64497  & 3.40278 \\
 1123 & 14457.2    &  70712.8  &  8.67442 &  1730.72 & 1.4338   & 6.14321 \\
 1168 &  4232.44   & 183953    & 14.5915  & 22840.3  & 0.734794 & 2.2048  \\
 1295 &  8518.29   & 143544    &  7.77065 &  4136.4  & 1.32589  & 5.49906 \\
\hline
\end{tabular}

==> false_positive_anchors.tex <==
\begin{tabular}{rlrr}
\hline
    & anchor                                                                                                             &   precision &   coverage \\
\hline
  0 & ['29899.00 \ensuremath{<} TVL \ensuremath{<}= 73782.70', '0.78 \ensuremath{<} OCR \ensuremath{<}= 1.45', '2027.60 \ensuremath{<} CSB \ensuremath{<}= 6400.19', 'CVD \ensuremath{<}= 6.38']                    &    0.767613 & 0.0300325  \\
  1 & ['TVL \ensuremath{>} 73782.70', 'CSB \ensuremath{>} 6400.19', 'HRT \ensuremath{<}= 5368.92', '0.50 \ensuremath{<} OCR \ensuremath{<}= 1.45']                                        &    0.818286 & 0.0819805  \\
  2 & ['29899.00 \ensuremath{<} TVL \ensuremath{<}= 73782.70', '2.95 \ensuremath{<} OHLR \ensuremath{<}= 4.92', 'OCR \ensuremath{>} 0.78', 'CSB \ensuremath{>} 477.28']                                &    0.772366 & 0.0503247  \\
  3 & ['TVL \ensuremath{>} 73782.70', '0.50 \ensuremath{<} OCR \ensuremath{<}= 1.45', '2.95 \ensuremath{<} OHLR \ensuremath{<}= 4.92', 'CSB \ensuremath{>} 6400.19']                                   &    0.891117 & 0.0178571  \\
  4 & ['29899.00 \ensuremath{<} TVL \ensuremath{<}= 73782.70', 'OHLR \ensuremath{<}= 2.95', '0.78 \ensuremath{<} OCR \ensuremath{<}= 1.45', 'HRT \ensuremath{<}= 5368.92', '2027.60 \ensuremath{<} CSB \ensuremath{<}= 6400.19'] &    0.767361 & 0.025974   \\
  5 & ['29899.00 \ensuremath{<} TVL \ensuremath{<}= 73782.70', '0.78 \ensuremath{<} OCR \ensuremath{<}= 1.45', 'CSB \ensuremath{<}= 6400.19', '2.95 \ensuremath{<} OHLR \ensuremath{<}= 4.92', 'CVD \ensuremath{>} 6.38']        &    0.900862 & 0.0146104  \\
  6 & ['TVL \ensuremath{>} 73782.70', '0.78 \ensuremath{<} OCR \ensuremath{<}= 1.45', 'CSB \ensuremath{>} 6400.19', 'CVD \ensuremath{<}= 6.38', '2.95 \ensuremath{<} OHLR \ensuremath{<}= 4.92']                    &    0.903042 & 0.00405844 \\
\hline
\end{tabular}

==> false_positives.tex <==
\begin{tabular}{rrrrrrr}
\hline
      &     HRT &      TVL &     CVD &      CSB &      OCR &    OHLR \\
\hline
   17 & 9022.53 &  63357.9 & 3.65344 &  2030.62 & 1.31047  & 5.29903 \\
  874 & 3824.17 &  86347.1 & 8.61754 &  9709.93 & 0.737519 & 2.57807 \\
  910 & 6041    &  73079.5 & 3.92434 &  1829.97 & 1.57896  & 4.73688 \\
  949 & 6470.73 & 145727   & 8.58034 & 12718.5  & 0.777694 & 3.38113 \\
 1041 & 4356.25 &  53523.4 & 7.80522 &  3820.21 & 1.03834  & 2.79306 \\
 1049 & 5704.43 &  55448.2 & 7.35395 &  3413.57 & 1.09367  & 3.04834 \\
 1180 & 7995.29 & 198886   & 5.61781 &  8527.49 & 1.41067  & 3.35659 \\
\hline
\end{tabular}

==> true_positive_anchors.tex <==
\begin{tabular}{rlrr}
\hline
    & anchor                                                                                                           &   precision &    coverage \\
\hline
  0 & ['TVL \ensuremath{>} 29899.00', 'OHLR \ensuremath{<}= 2.12', 'HRT \ensuremath{<}= 3365.87', 'OCR \ensuremath{>} 0.50', 'CVD \ensuremath{<}= 6.38']                                &    0.954545 & 0.0462662   \\
  1 & ['HRT \ensuremath{<}= 1323.51', 'CVD \ensuremath{>} 3.51', '0.78 \ensuremath{<} OCR \ensuremath{<}= 1.45']                                                           &    0.975    & 0.0219156   \\
  2 & ['TVL \ensuremath{>} 29899.00', 'HRT \ensuremath{<}= 3365.87', '0.50 \ensuremath{<} OCR \ensuremath{<}= 1.45', 'CSB \ensuremath{>} 477.28', '2.95 \ensuremath{<} OHLR \ensuremath{<}= 4.92', 'CVD \ensuremath{<}= 6.38'] &    0.923554 & 0.00405844  \\
  3 & ['TVL \ensuremath{>} 29899.00', 'HRT \ensuremath{<}= 3365.87', 'OCR \ensuremath{>} 0.50', 'CSB \ensuremath{>} 2027.60', 'CVD \ensuremath{<}= 3.51', 'OHLR \ensuremath{<}= 2.95']               &    0.985782 & 0.0202922   \\
  4 & ['HRT \ensuremath{<}= 1323.51', 'CVD \ensuremath{>} 3.51', 'TVL \ensuremath{<}= 29899.00', '0.50 \ensuremath{<} OCR \ensuremath{<}= 1.45', 'OHLR \ensuremath{<}= 2.95', 'CSB \ensuremath{>} 477.28']        &    0.962264 & 0.025974    \\
  5 & ['HRT \ensuremath{<}= 1323.51', 'CSB \ensuremath{>} 2027.60', '0.50 \ensuremath{<} OCR \ensuremath{<}= 0.78']                                                        &    0.961538 & 0.0714286   \\
  6 & ['HRT \ensuremath{<}= 1323.51', 'CVD \ensuremath{>} 6.38', 'OCR \ensuremath{<}= 1.45']                                                                  &    0.980861 & 0.0600649   \\
  7 & ['TVL \ensuremath{>} 29899.00', 'OHLR \ensuremath{<}= 2.12', 'HRT \ensuremath{<}= 3365.87', '0.50 \ensuremath{<} OCR \ensuremath{<}= 0.78', 'CSB \ensuremath{>} 2027.60']                      &    0.907975 & 0.0633117   \\
  8 & ['HRT \ensuremath{<}= 1323.51', 'CVD \ensuremath{>} 6.38']                                                                                 &    0.950199 & 0.0600649   \\
  9 & ['TVL \ensuremath{>} 73782.70', 'OHLR \ensuremath{<}= 2.12', 'CVD \ensuremath{<}= 6.38', 'OCR \ensuremath{>} 0.50']                                                  &    0.975    & 0.0146104   \\
 10 & ['TVL \ensuremath{>} 73782.70', '2.95 \ensuremath{<} OHLR \ensuremath{<}= 4.92', '0.78 \ensuremath{<} OCR \ensuremath{<}= 1.45', 'CSB \ensuremath{>} 2027.60']                                 &    0.87276  & 0.0275974   \\
 11 & ['HRT \ensuremath{<}= 1323.51', 'CSB \ensuremath{>} 2027.60', '0.50 \ensuremath{<} OCR \ensuremath{<}= 0.78']                                                        &    0.97479  & 0.0714286   \\
 12 & ['HRT \ensuremath{<}= 1323.51', 'CVD \ensuremath{>} 6.38', 'OCR \ensuremath{>} 0.50']                                                                   &    0.957746 & 0.0462662   \\
 13 & ['29899.00 \ensuremath{<} TVL \ensuremath{<}= 73782.70', '0.50 \ensuremath{<} OCR \ensuremath{<}= 0.78', 'HRT \ensuremath{<}= 5368.92', 'CSB \ensuremath{>} 6400.19', '2.95 \ensuremath{<} OHLR \ensuremath{<}= 4.92']   &    0.892116 & 0.000811688 \\
 14 & ['HRT \ensuremath{<}= 1323.51', 'CSB \ensuremath{>} 2027.60', '0.50 \ensuremath{<} OCR \ensuremath{<}= 1.45']                                                        &    0.955145 & 0.0917208   \\
 15 & ['TVL \ensuremath{>} 29899.00', 'HRT \ensuremath{<}= 3365.87', 'CSB \ensuremath{>} 6400.19', '0.78 \ensuremath{<} OCR \ensuremath{<}= 1.45', 'CVD \ensuremath{<}= 6.38', 'OHLR \ensuremath{<}= 4.92']       &    0.962567 & 0.00649351  \\
 16 & ['TVL \ensuremath{>} 29899.00', 'HRT \ensuremath{<}= 3365.87', 'OCR \ensuremath{>} 0.50', 'CSB \ensuremath{>} 2027.60', 'CVD \ensuremath{<}= 3.51']                               &    0.974522 & 0.0202922   \\
 17 & ['HRT \ensuremath{<}= 1323.51', 'CVD \ensuremath{>} 6.38', 'OCR \ensuremath{<}= 1.45']                                                                  &    0.962963 & 0.0600649   \\
 18 & ['HRT \ensuremath{<}= 1323.51', 'CSB \ensuremath{>} 6400.19', 'OCR \ensuremath{>} 0.50']                                                                &    0.984663 & 0.0478896   \\
 19 & ['HRT \ensuremath{<}= 1323.51', 'CSB \ensuremath{>} 6400.19', 'TVL \ensuremath{>} 73782.70', 'OCR \ensuremath{<}= 1.45']                                             &    0.972332 & 0.0162338   \\
 20 & ['TVL \ensuremath{>} 29899.00', 'HRT \ensuremath{<}= 1323.51', 'OCR \ensuremath{>} 0.50', 'CVD \ensuremath{>} 6.38']                                                 &    1        & 0.0349026   \\
 21 & ['HRT \ensuremath{<}= 1323.51', 'CVD \ensuremath{>} 6.38']                                                                                 &    0.954545 & 0.0600649   \\
 22 & ['TVL \ensuremath{>} 73782.70', '2.95 \ensuremath{<} OHLR \ensuremath{<}= 4.92', '2027.60 \ensuremath{<} CSB \ensuremath{<}= 6400.19', 'OCR \ensuremath{>} 0.50', 'CVD \ensuremath{>} 6.38']                &    0.802115 & 0.0162338   \\
 23 & ['TVL \ensuremath{>} 73782.70', '0.78 \ensuremath{<} OCR \ensuremath{<}= 1.45', 'CSB \ensuremath{>} 6400.19', '2.95 \ensuremath{<} OHLR \ensuremath{<}= 4.92']                                 &    0.921371 & 0.012987    \\
 24 & ['HRT \ensuremath{<}= 1323.51', 'CVD \ensuremath{>} 6.38']                                                                                 &    0.95664  & 0.0600649   \\
 25 & ['HRT \ensuremath{<}= 1323.51', 'CVD \ensuremath{>} 6.38', 'OCR \ensuremath{<}= 1.45']                                                                  &    0.96846  & 0.0600649   \\
 26 & ['TVL \ensuremath{>} 73782.70', '2.95 \ensuremath{<} OHLR \ensuremath{<}= 4.92', '2027.60 \ensuremath{<} CSB \ensuremath{<}= 6400.19', 'OCR \ensuremath{>} 0.50', 'CVD \ensuremath{>} 6.38']                &    0.748375 & 0.0162338   \\
 27 & ['HRT \ensuremath{<}= 1323.51', 'CSB \ensuremath{>} 2027.60', 'OCR \ensuremath{>} 0.50']                                                                &    0.950935 & 0.0917208   \\
 28 & ['HRT \ensuremath{<}= 1323.51', 'CSB \ensuremath{>} 6400.19', 'OCR \ensuremath{>} 0.50']                                                                &    0.988827 & 0.0478896   \\
 29 & ['HRT \ensuremath{<}= 1323.51', 'CSB \ensuremath{>} 6400.19', 'OCR \ensuremath{>} 0.50']                                                                &    0.976401 & 0.0478896   \\
 30 & ['TVL \ensuremath{>} 29899.00', '0.50 \ensuremath{<} OCR \ensuremath{<}= 1.45', 'OHLR \ensuremath{>} 2.95', 'CSB \ensuremath{>} 2027.60', 'HRT \ensuremath{<}= 5368.92', 'CVD \ensuremath{<}= 6.38']        &    0.923274 & 0.0113636   \\
 31 & ['TVL \ensuremath{>} 73782.70', 'HRT \ensuremath{<}= 3365.87', 'OHLR \ensuremath{<}= 2.12', 'CVD \ensuremath{<}= 6.38']                                              &    0.954198 & 0.0227273   \\
 32 & ['TVL \ensuremath{>} 73782.70', '0.78 \ensuremath{<} OCR \ensuremath{<}= 1.45', '2.95 \ensuremath{<} OHLR \ensuremath{<}= 4.92', 'CSB \ensuremath{>} 6400.19']                                 &    0.901639 & 0.012987    \\
 33 & ['TVL \ensuremath{>} 73782.70', 'OHLR \ensuremath{<}= 2.12', 'HRT \ensuremath{<}= 3365.87', 'OCR \ensuremath{>} 0.50', 'CSB \ensuremath{>} 2027.60']                              &    0.972851 & 0.0251623   \\
 34 & ['HRT \ensuremath{<}= 1323.51', 'CVD \ensuremath{>} 6.38']                                                                                 &    0.967213 & 0.0600649   \\
 35 & ['HRT \ensuremath{<}= 1323.51', 'CSB \ensuremath{>} 6400.19', 'TVL \ensuremath{>} 73782.70']                                                            &    0.986971 & 0.0162338   \\
 36 & ['HRT \ensuremath{<}= 1323.51', 'CSB \ensuremath{>} 6400.19', 'OCR \ensuremath{>} 0.50']                                                                &    0.977728 & 0.0478896   \\
 37 & ['TVL \ensuremath{>} 73782.70', 'OHLR \ensuremath{<}= 2.12', 'HRT \ensuremath{<}= 3365.87', 'CVD \ensuremath{<}= 6.38']                                              &    0.952218 & 0.0227273   \\
 38 & ['HRT \ensuremath{<}= 1323.51', 'CSB \ensuremath{>} 6400.19', 'TVL \ensuremath{>} 73782.70']                                                            &    0.979351 & 0.0162338   \\
\hline
\end{tabular}

==> true_positives.tex <==
\begin{tabular}{rrrrrrr}
\hline
      &      HRT &      TVL &      CVD &      CSB &      OCR &    OHLR \\
\hline
   19 & 2609.82  &  52097.8 &  3.95927 &  8040.03 & 0.638311 & 2.11822 \\
   66 &  441.55  &  17639.1 &  3.75271 &  1516.4  & 1.044    & 2.28086 \\
   73 & 3109.93  &  35831.7 &  3.76063 &  1994.3  & 1.0851   & 3.39273 \\
   87 & 2313.13  &  34666.3 &  2.67487 &  3613.87 & 0.78219  & 2.62175 \\
  105 &  218.46  &  11421.8 &  4.22215 &  1499.51 & 0.759894 & 2.03043 \\
  106 &  405.339 &  17068.2 &  2.54938 &  3112.34 & 0.622723 & 1.78129 \\
  697 &  300.632 &  25288   &  8.53431 &  2869.42 & 0.808995 & 1.99394 \\
  727 & 1584.77  &  72973.4 & 11.3611  &  9270.87 & 0.77715  & 2.01089 \\
  739 & 1029.37  &  53644.9 &  6.89909 & 30557.2  & 0.263416 & 1.84914 \\
  742 & 1347.77  &  77778   &  4.62887 & 14301.8  & 0.687641 & 1.56219 \\
  751 & 6270.17  &  95865.6 & 13.1038  &  4530.5  & 1.15049  & 3.87294 \\
  796 &  288.927 &  21172.9 &  2.69144 &  2937.96 & 0.71097  & 2.08576 \\
  828 & 1192.78  &  61388.4 &  9.26951 & 11610.7  & 0.561828 & 2.02027 \\
  881 & 4061.22  &  69100.1 & 45.7168  &  9250.92 & 0.58797  & 3.19523 \\
  885 &  202.222 &  15570.8 &  5.77785 &  2658.06 & 0.64074  & 1.84766 \\
  893 & 2731.53  &  73553.7 &  3.6388  &  8554.17 & 0.798341 & 2.20317 \\
  907 & 2510.42  &  66858.1 &  3.04159 &  5863.1  & 0.991266 & 2.27641 \\
  926 &  345.006 &  23287.8 &  6.54853 &  3235.2  & 0.699292 & 2.09231 \\
  942 & 1273.4   &  68874.1 &  5.47434 &  8034.04 & 0.853318 & 2.00982 \\
  962 & 1300.01  & 116883   &  3.81305 & 53383.7  & 0.334605 & 1.5425  \\
  977 &  813.865 &  52134.7 & 21.7931  &  6583.38 & 0.711397 & 2.25569 \\
  979 &  974.464 &  53841.2 & 17.4889  &  3656.64 & 1.2191   & 2.43655 \\
  983 & 8069.45  & 125770   & 13.0288  &  4027.15 & 1.57955  & 3.89814 \\
 1025 & 6318.91  & 100544   &  8.74434 &  6966.94 & 0.918667 & 3.39906 \\
 1029 &  791.968 &  43335.2 & 24.9265  & 13887.6  & 0.384082 & 1.89445 \\
 1031 &  910.602 &  51342.3 & 15.7182  &  9119.15 & 0.537392 & 2.25882 \\
 1035 & 8576.46  & 109602   &  9.07492 &  3646.48 & 1.50985  & 4.12691 \\
 1044 &  763.677 &  26957.8 &  3.08956 &  3665.52 & 0.69792  & 2.14417 \\
 1061 &  749.821 &  30970.3 &  4.80222 &  6990.88 & 0.55524  & 1.60327 \\
 1102 &  951.637 &  33192.9 &  4.36761 &  7543.69 & 0.510477 & 1.77904 \\
 1152 & 3912.31  &  42573.1 &  5.89289 &  3004.97 & 0.950434 & 3.06784 \\
 1174 & 2105.13  & 156918   &  5.31084 & 26974.6  & 0.675596 & 1.72263 \\
 1198 & 7421.48  & 179763   & 10.928   & 12115.2  & 0.927617 & 3.38255 \\
 1207 & 1919.11  & 106585   & 21.6469  & 17310.2  & 0.634051 & 1.99353 \\
 1220 & 1198.19  &  78843   & 11.1604  &  8581.75 & 0.844376 & 2.17303 \\
 1221 &  991.979 & 104671   &  4.60595 & 43708.5  & 0.434224 & 1.13433 \\
 1222 & 1322.37  & 100761   &  4.45947 & 14718.8  & 0.750554 & 1.83267 \\
 1263 & 1439.24  & 100558   &  3.51522 & 13145.5  & 0.813175 & 1.86599 \\
 1276 &  963.071 &  96033.2 &  4.62774 & 41389.6  & 0.378288 & 1.31964 \\
\hline
\end{tabular}
